Recipe: Hardware-Accelerated Replication Protocols

Replication protocols are essential for distributed systems, ensuring consistency, reliability, and fault tolerance. Traditional Crash Fault Tolerant (CFT) protocols, which assume a fail-stop model, are inadequate for untrusted cloud environments where adversaries or software bugs can cause Byzantine behavior. Byzantine Fault Tolerant (BFT) protocols address these threats but face significant performance, resource overheads, and scalability challenges. This paper introduces Recipe, a novel approach to transforming CFT protocols to operate securely in Byzantine settings without altering their core logic. Recipe rethinks CFT protocols in the context of modern cloud hardware, including many-core servers, RDMA-capable networks, and Trusted Execution Environments (TEEs). The approach leverages these advancements to enhance the security and performance of replication protocols in untrusted cloud environments. Recipe implements two practical security mechanisms, i.e., transferable authentication and non-equivocation, using TEEs and high-performance networking stacks (e.g., RDMA, DPDK). These mechanisms ensure that any CFT protocol can be transformed into a BFT protocol, guaranteeing authenticity and non-equivocation. The Recipe protocol consists of five key components: transferable authentication, initialization, normal operation, view change, and recovery phases. The protocol's correctness is formally verified using Tamarin, a symbolic model checker. Recipe is implemented as a library and applied to transform four widely used CFT protocols-Raft, Chain Replication, ABD, and AllConcur-into Byzantine settings. The results demonstrate up to 24x higher throughput compared to PBFT and 5.9x better performance than state-of-the-art BFT protocols. Additionally, Recipe requires fewer replicas and offers confidentiality, a feature absent in traditional BFT protocols.

==> abstract-old.tex <==
% \if 0
% \begin{abstract}
% Distributed data stores predominantly deploy replication protocols for fault tolerance and improved read-heavy performance. More specifically, Crash Fault Tolerant (CFT) replication protocols maintain a consistent view of their state among the replicas and guarantee availability in the face of failures. As we are moving to untrusted third-party cloud environments, nodes might fail arbitrarily due to configuration errors, bugs, malicious attacks, etc. Unfortunately, CFT protocols cannot guarantee correctness in the face of these non-benign faults.

% While Byzantine Fault Tolerant (BFT) protocols can handle arbitrary failures, BFT replication is very expensive, complex and hard to understand. Our work addresses these limitations by hardening the properties of CFT protocols to tolerate Byzantine faults. Specifically, we realize synergies between recent advances in hardware (trusted computing and networking) and BFT and we ask the following question: \emph{Can we leverage (and how) the state-of-the-art trusted hardware and networking to build a transformation of a CFT protocol for Byzantine settings while offering performance?}

% To answer the question we propose \projecttitle{}, a generic approach to transform CFT protocols to tolerate Byzantine failures. \projecttitle{} leverages the advances in Trusted Execution Environments and direct network I/O to guarantee non-equivocation and  authentication in the presence of Byzantine actors offering performance and generality. Our evaluation against PBFT and Damysus (a derivative of HotStuff) shows that \projecttitle{} can increase throughput up to $24\times$ and up to $5.9\times$, respectively, while decreasing the number of replicas by $f$ (w.r.t. PBFT). Lastly, \projecttitle{} can also provide confidentiality---a property not provided by conventional BFT protocols---with a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.


% \end{abstract}
% \fi

\begin{abstract}

Distributed systems ubiquitously rely on Crash Fault Tolerance (CFT) replication protocols for performance when (benign) faults occur. Unfortunately, CFT protocols are {\em inadequate} for modern untrusted cloud environments, where the underlying cloud infrastructure can be compromised by an adversary and fail in arbitrary ways (Byzantine failures). %, e.g., co-located tenants or even a misbehaving cloud operator. 
% %that may eavesdrop or actively influence the replicas' behavior
% To overcome these limitations,



%we investigate the impact of
%modern hardware on the performance of strongly-consistent
%replication protocols.

%Byzantine Fault Tolerant (BFT) protocols lay the foundations for maintaining a consistent view of the distributed state among the replicas and guaranteeing availability, {\em even in the presence of malicious adversaries}. While BFT protocols can tolerate arbitrary (Byzantine) failures, they are unfortunately {\em not adopted in practice} because of their high-performance overheads, replication resource overheads, and implementation complexity. 

%Our work addresses these BFT limitations by exploring the impact of modern hardware on the security and performance of strongly consistent replication protocols. Specifically, we target the following question:  

%we realize the synergies between the recent advances in the cloud hardware (trusted computing for confidential computing and RDMA-based/kernel-bypass networking) and replication protocols \manos{Until this point, this paragraph is very vague}: 

Today’s modern hardware, with manycore servers, RDMA-capable networks and trusted execution environments, challenges the conventional wisdom on CFT
protocol design. In this paper, we explore the synergy between modern hardware and the security and performance of strongly consistent replication protocols. In other words, \emph{can we leverage (and how) modern cloud hardware to harden the security properties of a CFT protocol for Byzantine settings while achieving high performance?}

To answer the question, we propose \projecttitle{}, a generic approach to transform {\em existing} CFT protocols to tolerate Byzantine failures in untrusted cloud environments. \projecttitle{} leverages the advances in confidential computing and direct network I/O to guarantee non-equivocation and transferable authentication in the presence of Byzantine actors while offering performance and resource overheads on par with CFT protocols. Importantly, \projecttitle{}'s APIs are generic and can easily be adapted to existing codebases---we have transformed a range of leader-/leaderless-based CFT protocols enforcing different (e.g., total order/per-key) ordering semantics.  Our evaluation based on the transformation of four CFT protocols (Raft, ABD, Chain Replication, and AllConcur) against the state-of-the-art BFT protocols shows that \projecttitle{} can increase throughput up to $5.9\times$---$24\times$, while requiring fewer replicas, i.e., 2$f$+1 replicas instead of 3$f$+1 replicas to tolerate $f$ faults. Lastly, we provide a correctness analysis for the safety and liveness properties of our transformation of CFT protocols operating in Byzantine settings. 


%PBFT and Damysus (a derivative of HotStuff) shows that \projecttitle{} can increase throughput up to $24\times$ and up to $5.9\times$, respectively, while decreasing the number of replicas by $f$ (w.r.t. PBFT). Lastly, \projecttitle{} can also provide confidentiality---a property not provided by conventional BFT protocols---with a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.


\end{abstract}

==> abstract.tex <==
% \if 0
% \begin{abstract}
% Distributed data stores predominantly deploy replication protocols for fault tolerance and improved read-heavy performance. More specifically, Crash Fault Tolerant (CFT) replication protocols maintain a consistent view of their state among the replicas and guarantee availability in the face of failures. As we are moving to untrusted third-party cloud environments, nodes might fail arbitrarily due to configuration errors, bugs, malicious attacks, etc. Unfortunately, CFT protocols cannot guarantee correctness in the face of these non-benign faults.

% While Byzantine Fault Tolerant (BFT) protocols can handle arbitrary failures, BFT replication is very expensive, complex and hard to understand. Our work addresses these limitations by hardening the properties of CFT protocols to tolerate Byzantine faults. Specifically, we realize synergies between recent advances in hardware (trusted computing and networking) and BFT and we ask the following question: \emph{Can we leverage (and how) the state-of-the-art trusted hardware and networking to build a transformation of a CFT protocol for Byzantine settings while offering performance?}

% To answer the question we propose \projecttitle{}, a generic approach to transform CFT protocols to tolerate Byzantine failures. \projecttitle{} leverages the advances in Trusted Execution Environments and direct network I/O to guarantee non-equivocation and  authentication in the presence of Byzantine actors offering performance and generality. Our evaluation against PBFT and Damysus (a derivative of HotStuff) shows that \projecttitle{} can increase throughput up to $24\times$ and up to $5.9\times$, respectively, while decreasing the number of replicas by $f$ (w.r.t. PBFT). Lastly, \projecttitle{} can also provide confidentiality---a property not provided by conventional BFT protocols---with a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.


% \end{abstract}
% \fi

\begin{abstract}

% Distributed data stores ubiquitously employ Crash Fault Tolerant (CFT) replication protocols for fault tolerance and performance. Unfortunately, CFT protocols are {\em inadequate} for modern untrusted cloud environments, since the underlying cloud infrastructure can be compromised by an adversary. %, e.g., co-located tenants or even a misbehaving cloud operator. 
% %that may eavesdrop or actively influence the replicas' behavior
% To overcome these limitations,

Byzantine Fault Tolerant (BFT) protocols lay the foundations for maintaining a consistent view of the distributed state among the replicas and guaranteeing availability, {\em even in the presence of malicious adversaries}. While BFT protocols can tolerate arbitrary (Byzantine) failures, they are unfortunately {\em not adopted in practice} because of their high-performance overheads, replication resource overheads, and implementation complexity. 

Our work addresses these BFT limitations by exploring the impact of modern hardware on the security and performance of strongly consistent replication protocols. Specifically, we target the following question:  
%we realize the synergies between the recent advances in the cloud hardware (trusted computing for confidential computing and RDMA-based/kernel-bypass networking) and replication protocols \manos{Until this point, this paragraph is very vague}: 
\emph{Can we leverage (and how) modern cloud hardware to harden the security properties of a Crash Fault Protocol (CFT) for Byzantine settings while achieving high performance?}

To answer the question, we propose \projecttitle{}, a generic approach to transform {\em existing} CFT protocols to tolerate Byzantine failures in untrusted cloud environments. \projecttitle{} leverages the advances in confidential computing and direct network I/O to guarantee non-equivocation and transferable authentication in the presence of Byzantine actors while offering performance and resource overheads on par with CFT protocols. Importantly, \projecttitle{}'s APIs are generic and can easily be adapted to existing codebases---we have transformed a range of leader-/leaderless-based CFT protocols enforcing different (e.g., total order/per-key) ordering semantics.  Our evaluation based on the transformation of four CFT protocols (Raft, ABD, Chain Replication, and AllConcur) against the state-of-the-art BFT protocols shows that \projecttitle{} can increase throughput up to $5.9\times$---$24\times$, while requiring fewer replicas, i.e., 2$f$+1 replicas instead of 3$f$+1 replicas to tolerate $f$ faults. Lastly, we provide a correctness analysis for safety and liveness properties of our transformation of CFT protocols operating in Byzantine settings. 


%PBFT and Damysus (a derivative of HotStuff) shows that \projecttitle{} can increase throughput up to $24\times$ and up to $5.9\times$, respectively, while decreasing the number of replicas by $f$ (w.r.t. PBFT). Lastly, \projecttitle{} can also provide confidentiality---a property not provided by conventional BFT protocols---with a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.


\end{abstract}

==> intro-PODC.tex <==
\section{Introduction}
\label{sec:introduction}

\myparagraph{}

\myparagraph{Motivation} Replication protocols play a foundational role in designing distributed data storage systems~\cite{10.14778/3007263.3007267, 10.14778/2002938.2002939, zippydb, bankDB, NetflixDB, GEDB, HESSDB}, distributed ledgers~\cite{baasAlibaba, baasAWS, baasAzure, baasIBM, baasOracle}, distributed data analytics systems~\cite{NetflixDB}. For performance and fault tolerance requirements, distributed systems employ Crash Fault Tolerant (CFT) {\em replication protocols}~\cite{raft,chain-replication, 10.5555/1855807.1855818, Reed2008AST, 10.5555/800253.807732, lynch:1997, 10.1145/279227.279229, Hermes:2020} to maintain a consistent view of the datasets guaranteeing fault tolerance, i.e., reliability and availability in the presence of failures~\cite{zippydb, dynamo, lakshman2009, redis, rocksdb, leveldb, memcached2004, bfthyperledger}.
%while improving the performance for read-heavy workloads and, more importantly,





Unfortunately, CFT protocols assume a {\em fail-stop model}\manos{It's a bit weird to say that a crash fault tolerant unfortunately only tolerates crash faults}, i.e., replicas are honest and can only fail by crashing~\cite{delporte}. As such, they are {\em inadequate} for modern untrusted cloud environments, where the underlying cloud infrastructure can be compromised by an adversary, e.g., co-located tenants or even a misbehaving cloud operator that may eavesdrop or actively influence the replicas' behavior\manos{Citations here? Some of the follow-up work to Foreshadow was showing that such attacks are possible, for example. Also, is eavesdropping relevant? That implies read-only access and doesn't affect the behavior of the system}. In such an untrusted environment, the surface of faults and attacks expands beyond the CFT fail-stop model, ranging from software bugs and configuration errors to malicious attacks~\cite{Gunawi_bugs-in-the-cloud, Shinde2016, hahnel2017high}. CFT protocols are fundamentally incapable of providing consistent replication in the presence of non-benign ({\em Byzantine}) faults in untrusted cloud environments.


bring 2.1 (BFT vsCFT)
\myparagraph{Limitations of state-of-the-art approaches}While Byzantine Fault Tolerant (BFT) protocols~\cite{Lamport:1982} offer important foundations for developing distributed systems with stronger guarantees in the presence of {\em Byzantine failures} (i.e., nodes can fail in arbitrary ways), they are {\em not adopted \underline{in practice}} because of their high-performance and replication resource overheads, and implementation complexity~\cite{visigoth-eurosys}.

The “CFT vs. BFT" conundrum creates a fundamental design trade-off between the {\em efficiency of CFT protocols} for practical deployments and the {\em robustness of BFT protocols} for Byzantine settings of modern cloud environments. However, traditional BFT protocols design and evaluation has not taken into account {\em modern cloud hardware}. 
 
%To overcome the limitations of  CFT protocols,  While BFT protocols can tolerate Byzantine failures, {\em including malicious adversaries}, they are unfortunately {\em not adopted in practice} because of their high-performance and replication resource overheads, and implementation complexity~\cite{visigoth-eurosys}. For instance, BFT protocols require $3f+1$ replicas instead of the $2f+1$ replicas required by CFT protocols for tolerating $f$ faults. BFT protocols also require additional communication rounds (at least three phases instead of two phases in the CFT model); thus incurring high latency and reduced read/write throughput. Lastly, BFT protocols are extremely complex and hard to understand, let alone to implement correctly and optimize~\cite{unsafeZyzzyva}: even intuitive algorithmic optimizations can strongly affect other parts of the protocol~\cite{10.1145/2658994}.

%While the “CFT vs. BFT" conundrum creates a fundamental design trade-off between the {\em efficiency of CFT protocols} for practical deployments and the {\em robustness of BFT protocols} for Byzantine settings of modern cloud environments. %To strike a balance, our work targets the following research question: {\em How can we design robust and efficient replication protocols for distributed systems hosted in untrusted cloud environments?}


bring 2.3

\myparagraph{Key insights and high-level design} Our work seeks to resolve this trade-off leveraging modern cloud hardware for transforming existing CFT protocols for Byzantine settings in untrusted cloud environments. Our transformation underpins the robustness and efficiency axes.
For {\em robustness}, we leverage trusted hardware available as part of confidential cloud computing to harden the security properties of CFT protocols~\cite{intel-sgx, keystone_eurosys, amd-sev, intelTDX}. In particular, we leverage trusted execution environments (TEEs) to provide two key properties for successfully transforming a CFT protocol to operate in Byzantine settings, as identified by Clement et al.~\cite{clement2012}: (a) transferable authentication, i.e., the ability to establish trust in nodes in distributed settings by designing a remote attestation protocol, and (b) non-equivocation, i.e., once the trust is established in a node via the remote attestation protocol, the node follows the CFT replication protocol faithfully, and therefore, it cannot send conflicting statements to other nodes. %to reach agreement in the presence of Byzantine faults in the asynchronous communication model.

For {\em efficiency}, we leverage the modern networking hardware, such as RDMA/DPDK for kernel bypass, to design a highly optimized communication protocol for replicating the state across nodes in distributed settings~\cite{rdma, dpdk, erpc}, while overcoming the I/O bottlenecks in trusted computing~\cite{rkt-io}.


-> Say that the theoretical transformation has not beeing realised


\myparagraph{Our proposal: \projecttitle{}} 
\projecttitle{} leverages TEEs along with direct I/O to resolve the tension between security and performance by building an efficient and practical transformation of unmodified CFT replication protocols for Byzantine settings. \projecttitle{} achieve this by implementing a distributed trusted computing base (TCB) that shields the replication protocol execution and {\em extends} the security properties offered by a single TEE (whose security properties are only effective in a single-node setup) to a distributed setting of TEEs. Our design is comprised of a transferable authentication phase ($\S$~\ref{sec:attestation}) for distributed trust establishment, a high-performant network stack for secure communication over the untrusted network ($\S$~\ref{subsec:networkin}) and a memory-efficient KV store ($\S$~\ref{subsec:KV}).  We materialise \projecttitle{} approach as a generic library, \projecttitle{}-lib ($\S$~\ref{sec:recipe-implementation}).


%We materialise \projecttitle{} approach as a generic library, \projecttitle{}-lib ($\S$~\ref{sec:recipe-implementation}), on top of Intel SGX and the \scone{} framework~\cite{arnautov2016scone}. We carefully build \projecttitle{}'s high-performance network stack for TEEs, extending eRPC~\cite{erpc} to enable direct I/O, essentially DMA operations, within the protected TEE domain while shielding the exchanged messages to maintain authenticity and non-equivocation accross the network. Lastly, our lock-free KV store is designed to optimize for the limited trusted area in TEEs~\cite{speicher-fast, shieldstore}.% on top of folly library~\cite{folly}.



Our evaluation assesses \projecttitle{}'s generality and efficiency. Specifically, to show the generality of our approach, we apply and evaluate \projecttitle{} on real hardware with four well-known CFT protocols (from now on, an `R-' prefix stands for the transformed protocol); a decentralized (leaderless) linearizable multi-writer multi-reader protocol (ABD)~\cite{lynch:1997} (R-ABD), two leader-based protocols with linearizable reads, Raft~\cite{raft} (R-Raft) and Chain Replication (CR)~\cite{chain-replication} (R-CR), and AllConcur~\cite{Poke2016AllConcurLC} (R-AllConcur), a decentralized consensus protocol with consistent local reads. To evaluate performance, we compare \projecttitle{} protocols with two competitive BFT replication protocols, BFT-smart~\cite{bft-smart} (PBFT~\cite{Castro2002}), whose specific implementation has been adopted in industry~\cite{bftsmarthyperledger} and Damysus~\cite{10.1145/3492321.3519568} a state-of-the-art BFT replication protocol.  Our evaluation shows that \projecttitle{} achieves up to $24\times$ and $5.9\times$ better throughput w.r.t. PBFT and Damysus, respectively, while improving scalability---\projecttitle{} requires $2f+1$ replicas, $f$ fewer replicas compared to PBFT ($3f+1$). We further show that \projecttitle{} can offer confidentiality---a security property not provided by traditional BFT protocols---while achieving a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.

%\myparagraph{Artifact} \projecttitle{} is available as an open-source project.%: \url{https://anonymous.4open.science/r/secure_replication-907F/}.


%build on top of Intel SGX. Our \projecttitle{} up to $24\times$ and $5.9\times$ better throughput w.r.t. BFT-smart and Damysus.
To summarize, we make the following contributions:

\begin{itemize}[leftmargin=*]
    \item {\bf Hardware-assisted transformation of CFT protocols:} We present \projecttitle{}, a generic approach for transforming CFT protocols to tolerate Byzantine failures without any modifications to the core of the protocols.%, e.g., states, message rounds, and complexity. %We realize our approach by implementing \projecttitle{}-lib leveraging the advances in modern hardware; we use trusted hardware to guarantee transferrable authentication and non-equivocation for thwarting Byzantine errors. Further, we combine trusted hardware with direct network I/O (RDMA/DPDK~\cite{rdma, dpdk}) for performance.

    \item {\bf Generic \projecttitle{} APIs:} We propose generic \projecttitle{} APIs to transform the existing codebase of CFT protocols for Byzantine settings. Using \projecttitle{} APIs, we have successfully
transformed a range of leader-/leaderless-based CFT protocols enforcing different ordering semantics. % We further show that \projecttitle{} can offer confidentiality---a security property not provided by traditional BFT protocols.

    
    \item {\bf Formal correctness analysis:}  We provide a correctness analysis for the safety and liveness properties of our
transformation of CFT protocols operating in Byzantine settings. % We provide a formal analysis showing the correctness and 
    \item {\bf \projecttitle{} in action:} We present an extensive evaluation of \projecttitle{} by applying it to four CFT protocols: Chain Replication, Raft, ABD, and AllConcur. We evaluate these four protocols against the state-of-the-art BFT protocol implementations and show that \projecttitle{} achieves up to $24\times$ and $5.9\times$ better throughput.
    
  %  BFT-smart~\cite{bft-smart}, an optimized version of PBFT~\cite{Castro:2002} and Damysus~\cite{10.1145/3492321.3519568}, an optimized version of HotStuff~\cite{DBLP:journals/corr/abs-1803-05069}. Our evaluation shows that \projecttitle{} achieves up to $24\times$ and $5.9\times$ better throughput w.r.t. PBFT and Damysus, respectively, while improving scalability---\projecttitle{} requires $2f+1$ replicas, $f$ fewer replicas compared to PBFT ($3f+1$). We further show that \projecttitle{} can offer confidentiality---a security property not provided by traditional BFT protocols---while achieving a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.
\end{itemize}


==> intro.tex <==
\section{Introduction}
\label{sec:introduction}
Our growing reliance on online services requires highly available, fast and trustworthy systems that remain correct even when failures occur. The vast majority of cloud services provide availability in the presence of faults by deploying Crash Fault Tolerant (CFT)  replication protocols. CFT protocols assume a fail-stop fault
model; the replicas are honest and can only fail by crashing~\cite{delporte}. However, the wide adoption of online services in the third-party untrusted cloud infrastructure has drastically increased the surface of faults and attacks that range from software bugs and configuration errors to malicious attacks~\cite{Gunawi_bugs-in-the-cloud, Shinde2016,hahnel2017high}. Unfortunately, CFT protocols are fundamentally incapable of providing consistent replication in the presence of non-benign faults.
%are insufficient to
%meet all the security properties required by a pplications hosted in the cloud.

\if 0
Indeed, recent research~\cite{Gunawi_bugs-in-the-cloud, Shinde2016,hahnel2017high} shows that malicious attackers are now able to get advantage of software bugs, configuration errors and security vulnerabilities and tamper with the properties and semantics of modern online applications (e.g., databases, KV stores, financial and banking applications, blockchain, etc.). 
All these arbitrary behaviors are modeled under the notion of the Byzantine Fault Model. 
\fi

On the other hand, Byzantine Fault Tolerance (BFT)~\cite{Lamport:1982} offers important foundations for developing protocols with stronger guarantees in the presence of Byzantine actors, i.e., processes that fail in arbitrary ways. %other than silently crashing. %Practical systems~\cite{bft-smart} that implement state machine replication have adopted this model to provide resiliency against arbitrary faults. 
%While BFT protocols (BFTs) target Byzantine settings where the nodes involved can behave arbitrarily and be dishonest, 
Unfortunately, traditional BFT protocols present severe limitations that impede their adoption in high-end distributed systems.
%Unfortunately, traditional BFT protocols present the following severe limitations with respect to high-end distributed systems. 
{\bf First}, BFT protocols are slow due to high message complexity (typically, $O(n^2)$) and multiple protocol rounds. {\bf Second}, they require at least $3f+1$ nodes to tolerate up to $f$ Byzantine nodes which severely limits scalability. In contrast, widely adopted CFT protocols~\cite{raft, Reed2008AST, primary-backup, engraft} comprise two rounds and $O(n)$ message complexity with $2f+1$ replicas.% \pramod{shall we contrast these costs wrt. CFT protocols?} ~\cite{Hunt:2010,etcd}, e.g., Raft

{\bf Finally}, BFT protocols are complex, introducing burdens to developers. Even if system designers wish to use a state-of-the-art BFT protocol, optimizing it for the specific application settings can be complicated. 
Guerraoui et al.~\cite{10.1145/2658994} found that most protocol implementations consist of thousands of lines of code, e.g., PBFT~\cite{Castro:2002} and Zyzzyva~\cite{10.1145/1658357.1658358}. Even trivial changes or intuitively simple modifications for optimizing for the common case, are extremely hard and might affect other parts of the protocol (e.g., view-change in Zyzzyva).

All the above in combination with the difficulty of testing distributed protocols~\cite{Chandra2007PaxosML} require great effort for designing and optimizing such protocols. Consequently, BFT protocols are still not widely adopted by cloud services~\cite{bft-time-is-now, 10.1145/1711475.1711494} that, instead, rely on CFT protocols to handle failures~\cite{Hunt:2010,etcd, zippy, 51, redis}.

%\pramod{should we make a point that because of these limitations BFT protocols are still not widely adopted when compared to CFT? The next para can have a transisition -- To overcome these limitations, previous works.}


%The only complete proof of a BFT protocol we knew of is that of PBFT and it involves 35 pages (even without using any formal language).1 This difficulty, together with the impossibility of exhaustively testing distributed protocols [8] would rather plead for never changing a protocol that was tested and proven correct, e.g., PBFT.

%on transforming current BFT protocols to CFT protocols by 
Previous works~\cite{minBFT, hybster, DBLP:journals/corr/LiuLKA16a, A2M, 10.1145/2168836.2168866} aim at optimizing BFT protocols and mostly focus on reducing the number of replicas required. They use trusted modules along with the protocol's ``traditional'' (untrusted) counterpart to prevent Byzantine processes from making conflicting statements for the same request (equivocation). As before, all of these efforts require programmers to understand, transform and optimize these complex protocols; a task that is quite challenging.%can rapidly turn into a nightmare.



%\myparagraph{{\bf Motivation}}


\if 0
%\begin{itemize}
%    \item[1.] BFT protocols are slow as they occur high message complexity (typically, $O(n^2)$) and multiple protocol rounds/phases (3PC). Further, they traditionally require at least $3f+1$ nodes for tolerating up to $f$ Byzantine nodes which greatly limits scalability.
%    \item[2.] BFT protocols do *not* target strong security properties---specifically confidentiality where only authorized nodes/clients can access the data~\cite{avocado}. In general, it would be safe to say that current BFT does not target a typical, yet realistic, security threat model~\cite{Baumann2014} where the third party cloud provider and infrastructure that hosts the application is untrusted.
%\item[3.] BFT is complex from the programmers perspective which introduces burdens to develop and optimize the protocol.
    %\item \underline{Solution}: Strong consistent CFT protocols \& TEEs
%\end{itemize}
\fi

\if 0
%Prior work~\cite{10.1145/2332432.2332490} formally defines two properties \emph{(i)} non-equivocation and \emph{(i)} transferable authentication and proves that these two properties are the lower bound for transforming a CFT protocol to a BFT protocol.


%We leverage the theory in~\cite{10.1145/2332432.2332490} and we go one step further designing, implementing and evaluating \projecttitle{}, an end-to-end library to systematically transform in practice CFTs to BFTs without further modifications on the process number, protocol rounds and messages complexity.
\fi

%In contrast to previous BFT$\rightarrow$CFT transformations, we go in the opposite direction and build a performance-efficient transformation of CFT protocols for Byzantine settings (CFT$\rightarrow$BFT) that allows designers to build protocols that tolerate Byzantine faults without having to become BFT experts.
In contrast to previous approaches that aim to minimize the number of replicas while offering BFT, we go in the opposite direction: we aim to harden the properties of CFT protocols building a performance-efficient transformation of CFT protocols for Byzantine settings (CFT$\rightarrow$BFT). Our transformation allows designers to build protocols that tolerate Byzantine faults without having to become BFT experts.


%We realize the potential of the recent advances in hardware---trusted computing and direct network I/O---and implement an efficient transformation, a ``\projecttitle{}'', of a CFT protocol for Byzantine settings. Our approach offers BFT while providing better performance than conventional BFT protocols. Note that CFT protocols require fewer nodes for availability, are well-documented and studied (both in research and production) and are easier to implement. 

We realize the potential of Trusted Execution Environments (TEEs) and implement an efficient transformation, a ``\projecttitle{}'', of a CFT protocol for Byzantine settings.  If used naively, however, TEEs incur great overheads~\cite{10.5555/1924943.1924946}. In this paper, we show how we can mitigate the performance impact of using TEEs by adopting direct network I/O. As a result, our approach offers BFT while providing {\em better performance than conventional BFT protocols} and reaping {\em all the benefits of CFT protocols} (fewer nodes, easier implementation, simplicity).
%like requiring fewer nodes for availability, being well-documented and studied, %and being easier to implement.

%Note that CFT protocols require fewer nodes for availability, are well-documented and studied (both in research and production) and are easier to implement. 


To sum up, this paper poses the following question: \emph{Can we leverage (and how) the advances in networking and trusted computing, like Trusted Execution Environments (TEEs) and direct I/O, to harden the properties of CFT protocols to (1) target a weaker fault model (i.e., Byzantine faults) while (2) offering performance and scalability?}  %However, they cannot target Byzantine settings out-of-the-box, as they assume a Fail/Crash fault model; the replicas are \emph{honest} and can only fail by crashing.
%; \emph{with TEEs we can guarantee \textbf{honesty} for the running application. As long as we have honesty, any malicious error can be ``seen'' as crash-stop behavior.} 

%\pramod{We intermix recipe as an approach and library
%6:39
%I think what can we say is the following:
%We present an approach -- recipe.
%Based on our approach, we build recipe-library which allows users to transform protocols %seamlessly.}

%Our answer to this question is positive. We support our claims by building \projecttitle{}, an end-to-end library that systematically transforms a CFT protocol~\cite{f04eb9b864204bab958e72055062748c} to handle Byzantine faults. \projecttitle{} is a generic library that prevents equivocation and guarantees authentication for the network. We leverage the state-of-the-art hardware to target both performance and BFT---two often contradictory notions; we use TEEs for trust and direct network I/O for performance.

Our answer is \projecttitle{}, an approach to transform a CFT protocol to handle Byzantine faults. We realize the \projecttitle{} approach as a generic library, \projecttitle{}-lib, that prevents equivocation and guarantees authentication for the network. Our key insight is the use of modern hardware to achieve both BFT and performance---two often contradictory goals; we use TEEs for trust and direct network I/O for performance.


%\pramod{the following pararaph can actually encapsulate all the implementation details under the "recipe libray". We build a generic library based on.., which allow...}
Our \projecttitle{}-lib, built on top of TEEs and direct network I/O, follows an established RPC-API, e.g., RDMA programming paradigm~\cite{rdma}, allowing system designers to seamlessly transform a CFT protocol for Byzantine settings. Although we make no assumptions about the TEE, we implement \projecttitle{}-lib on top of Intel SGX~\cite{intel-sgx} and \scone{}~\cite{arnautov2016scone}. In addition, we extend eRPC~\cite{erpc} (on top of DPDK~\cite{dpdk}) and we build a shielded high-performant networking library, carefully designed for TEEs, that preserves non-equivocation and authentication in the untrusted network.


To show the generality of \projecttitle{}, we apply and evaluate it on real hardware with four well-known CFT protocols (from now on `R-' prefix stands for the transformed protocol); a decentralized (leaderless) linearizable multi-writer multi-reader protocol (ABD)~\cite{lynch:1997} (R-ABD), two leader-based protocols with linearizable reads, Raft~\cite{raft} (R-Raft) and Chain Replication (CR)~\cite{chain-replication} (R-CR), and AllConcur~\cite{Poke2016AllConcurLC} (R-AllConcur), a decentralized consensus protocol with consistent local reads. %We build and evaluate these protocols with \projecttitle{} on real hardware. 

To sum up, we make the following contributions:


\begin{itemize}
    \item We present \projecttitle{}, a generic approach for transforming CFT protocols to tolerate Byzantine failures without any modifications to the protocols, e.g., states, message rounds and complexity.
    \item We realize our approach by implementing \projecttitle{}-lib leveraging the advances in modern hardware; specifically, we use Trusted Execution Environments (TEEs) to guarantee trust for the executed code and eliminate Byzantine errors. Further, we combine TEEs and direct network I/O (RDMA/DPDK~\cite{rdma, dpdk}) for performance.
    \item We provide proofs of correctness and we show the generality of \projecttitle{} by applying it to four CFT protocols.
    \item Lastly, we evaluate these four protocols against BFT-smart~\cite{bft-smart}, an optimized version of PBFT~\cite{Castro:2002} and Damysus~\cite{10.1145/3492321.3519568}, a transformed \addition{(using TEEs)} version of Hotstuff~\cite{DBLP:journals/corr/abs-1803-05069} with $2f+1$ replicas. Our evaluation shows that \projecttitle{} achieves up to $24\times$ and $5.9\times$ better throughput w.r.t. PBFT and Damysus, respectively, while improving scalability---\projecttitle{} requires $2f+1$ replicas, $f$ fewer replicas compared to PBFT ($3f+1$). We further show that \projecttitle{} can offer confidentiality---a security property not provided by traditional BFT protocols---while achieving a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.
\end{itemize}


\if 0
\begin{itemize}
    \item We show that a non-equivocation and integrity verification layer, jointly with TEEs, are necessary to transform a strong consistent CFT protocol to handle BFT settings. 
    \item We build \projecttitle{} which systematically transforms strong consistent CFT protocols to handle Byzantine errors without further modifications on the number of processes, protocol rounds and messages complexity. Our \projecttitle{} targets practical systems; we build three TEE-assisted primitives, i.e., non-equivocation, authentication and attestation, to harden the CFT protocols.
    \item We build \projecttitle{} leveraging the modern hardware trends on TEE and user-space networking, emphasizing on performance.
    \item We build and evaluate three widely adopted CFT protocols, R-ABD (\projecttitle{}'s derivative of ABD~\cite{lynch:1997}), R-Raft~\cite{raft}(\projecttitle{}'s derivative of Raft~\cite{raft}), and R-CR (\projecttitle{}'s derivative of CR~\cite{chain-replication}). Our evaluation of these three systems against BFT-smart~\cite{bft-smart} shows that we can achieve up to $100\times$ better throughput.
\end{itemize}

\dimitra{
Contributions:
\begin{itemize}
    \item We use modern software/hardware trends, i.e., Trusted Execution Environments, kernel by-pass networking (DPDK, RDMA, etc.) to offer \projecttitle{}, a powerful API to transform any Crash Fault Tolerant protocol to Byzantine Fault Tolerant settings.
    \item We offer a analysis of the correctness properties of \projecttitle{} (todos: check with Manos here).
    \item We offer an evaluation of four CFT protocols compared to BFT .. .
\end{itemize}
}
\fi
\if 0
\myparagraph{Key insight} While prior work has explored the synergies between TEEs and BFT protocols~\cite{A2M, minBFT} to prevent equivocation, we go one step further. Our key insight is the following: \emph{With TEEs we can guarantee \textbf{honesty} for the application running inside the enclave. As long as we have honesty, any malicious error can be ``seen'' as crash-stop behavior.}

\myparagraph{Solution} \projecttitle{} presents a recipe on how to systematically secure strong consistent CFT protocols~\cite{f04eb9b864204bab958e72055062748c} leveraging TEEs to achieve Byzantine settings tolerance. While BFT allows nodes to go out of spec, we leverage TEEs to build \projecttitle{} that disallows any node to go out of spec.

\myparagraph{Contributions}
\begin{itemize}
    \item We show that a non-equivocation and integrity verification layer, jointly with TEEs, are enough to transform a strong consistent CFT protocol to handle BFT settings. 
    \item We build \projecttitle{} which systematically transforms strong consistent CFT protocols to handle Byzantine errors without further modifications on the number of processes, protocol rounds and messages complexity. Our \projecttitle{} targets practical systems; we build three TEE-assisted primitives.
    \item We build \projecttitle{} leveraging the modern trends on Trusted execution environments and networking, emphasizing on performance.
    \item We build and evaluate three practical, widely adopted CFT protocols, ABD~\cite{}, Raft~\cite{raft}, Chain Replication~\cite{chain-replication} with \projecttitle{}. Our evaluation against PBFT-smart~\cite{bft-smart} shows that we can achieve ....
\end{itemize}
\fi

==> intro2.tex <==
\section{Introduction}
\label{sec:introduction}
Our growing reliance on online services requires highly available, fast and trustworthy systems that remain correct even when failures occur. The vast majority of cloud services provide availability in the presence of faults by deploying Crash Fault Tolerant (CFT)  replication protocols. CFT protocols assume a fail-stop fault
model; the replicas are honest and can only fail by crashing~\cite{delporte}. However, the wide adoption of online services in the third-party untrusted cloud infrastructure has drastically increased the surface of faults and attacks that range from software bugs and configuration errors to malicious attacks~\cite{Gunawi_bugs-in-the-cloud, Shinde2016, hahnel2017high}. Unfortunately, CFT protocols are fundamentally incapable of providing consistent replication in the presence of non-benign faults.


On the other hand, Byzantine Fault Tolerance (BFT)~\cite{Lamport:1982} offers important foundations for developing protocols with stronger guarantees in the presence of Byzantine actors, i.e., processes that fail in arbitrary ways. Unfortunately, traditional BFT protocols present severe limitations that impede their adoption in modern, high-end distributed systems. 

\noindent{\bf {\#1: Performance and scalability.}} BFT protocols are slow due to high message complexity (typically, $O(n^2)$) and multiple protocol rounds while they require at least $3f+1$ nodes to tolerate up to $f$ Byzantine nodes which severely limits scalability. In contrast, widely adopted CFT protocols~\cite{raft, Reed2008AST, primary-backup, engraft} comprise two rounds and $O(n)$ message complexity with $2f+1$ replicas.


\noindent{\bf {\#2: Complexity and adoption.}} BFT protocols are complex, introducing burdens to developers. Even if system designers wish to use a state-of-the-art BFT protocol, optimizing it for the specific application settings can be complicated. Guerraoui et al.~\cite{10.1145/2658994} found that most protocol implementations consist of thousands of lines of code, e.g., PBFT~\cite{Castro:2002} and Zyzzyva~\cite{10.1145/1658357.1658358}. Even trivial changes or intuitively simple modifications for optimizing for the common case, are extremely hard and might affect other parts of the protocol (e.g., view-change in Zyzzyva).


Previous research~\cite{minBFT, hybster, DBLP:journals/corr/LiuLKA16a, A2M, 10.1145/2168836.2168866} made an effort to optimize such protocols by reducing the number of replicas required with trusted hardware. They use trusted modules along with the protocol's ``traditional'' (untrusted) counterpart to prevent Byzantine processes from making conflicting statements for the same request (equivocation). As before, all of these efforts require programmers to understand, transform and optimize such complex protocols; a task that is quite challenging. As an evidence of this, BFT protocols are still not widely adopted by cloud services~\cite{bft-time-is-now, 10.1145/1711475.1711494} that, instead, sacrifice security and rely on CFT protocols to handle failures~\cite{Hunt:2010, etcd, zippy, redis, rafthyperledger}.

%%%All the above in combination with the difficulty of testing distributed protocols~\cite{Chandra2007PaxosML} require great effort for designing and optimizing such protocols. Consequently, BFT protocols are still not widely adopted by cloud services~\cite{bft-time-is-now, 10.1145/1711475.1711494} that, instead, rely on CFT protocols to handle failures~\cite{Hunt:2010,etcd, zippy, 51, redis}.



%The only complete proof of a BFT protocol we knew of is that of PBFT and it involves 35 pages (even without using any formal language).1 This difficulty, together with the impossibility of exhaustively testing distributed protocols [8] would rather plead for never changing a protocol that was tested and proven correct, e.g., PBFT.

%%%%% Previous works~\cite{minBFT, hybster, DBLP:journals/corr/LiuLKA16a, A2M, 10.1145/2168836.2168866} aim at optimizing BFT protocols and mostly focus on reducing the number of replicas required. They use trusted modules along with the protocol's ``traditional'' (untrusted) counterpart to prevent Byzantine processes from making conflicting statements for the same request (equivocation). As before, all of these efforts require programmers to understand, transform and optimize these complex protocols; a task that is quite challenging.



\noindent{\bf {Key insights, contributions and high-level design.}} In contrast to previous approaches that merely aim to minimize the number of replicas while offering BFT, we go in the opposite direction targeting both limitations at once: we aim to harden the properties of CFT protocols building a performance-efficient transformation of CFT protocols for Byzantine settings (CFT$\rightarrow$BFT). In addition, we show that our transformation can \emph{transparently} offer confidentiality to applications when they need it~\cite{ciad} ($\S$~\ref{sec:motivation}), an extra property not offered by traditional BFT, without sacrificing performance. More importantly, we give system designers the opportunity to build protocols that tolerate Byzantine faults without having to become BFT experts.


%We realize the potential of the recent advances in hardware---trusted computing and direct network I/O---and implement an efficient transformation, a ``\projecttitle{}'', of a CFT protocol for Byzantine settings. Our approach offers BFT while providing better performance than conventional BFT protocols. Note that CFT protocols require fewer nodes for availability, are well-documented and studied (both in research and production) and are easier to implement. 

We realize the potential of Trusted Execution Environments (TEEs) and implement an efficient transformation, a ``\projecttitle{}'', of a CFT protocol for Byzantine settings.  If used naively, however, TEEs incur great overheads~\cite{10.5555/1924943.1924946}. In this paper, we show how we can mitigate the performance impact of using TEEs by adopting direct network I/O. As a result, our approach offers BFT while providing {\em better performance (and security, i.e., confidentiality) than conventional BFT protocols} and reaping {\em all the benefits of CFT protocols} (fewer nodes, easier implementation, simplicity).

To sum up, this paper poses the following question: \emph{Can we leverage (and how) the advances in networking and trusted computing, like Trusted Execution Environments (TEEs) and direct I/O, to harden the properties of CFT protocols to (1) target a weaker fault model (i.e., Byzantine faults) while (2) offering performance and scalability?}

Our answer is \projecttitle{}, an approach to transform a CFT protocol to handle Byzantine faults. We realize the \projecttitle{} approach as a generic library, \projecttitle{}-lib, that prevents equivocation and guarantees authentication for the network. Our key insight is the use of modern hardware to achieve both BFT and performance---two often contradictory goals; we use TEEs for trust and direct network I/O for performance.


Our \projecttitle{}-lib, built on top of TEEs and direct network I/O, follows an established RPC-API, e.g., RDMA programming paradigm~\cite{rdma}, allowing system designers to seamlessly transform a CFT protocol for Byzantine settings. We implement \projecttitle{}-lib on top of Intel SGX~\cite{intel-sgx} and \scone{}~\cite{arnautov2016scone}. In addition, we extend eRPC~\cite{erpc} (on top of DPDK~\cite{dpdk}) and we build a shielded high-performant RPC library, carefully designed for TEEs, that preserves non-equivocation and authentication in the untrusted network.


To show the generality of \projecttitle{}, we apply and evaluate it on real hardware with four well-known CFT protocols (from now on `R-' prefix stands for the transformed protocol); a decentralized (leaderless) linearizable multi-writer multi-reader protocol (ABD)~\cite{lynch:1997} (R-ABD), two leader-based protocols with linearizable reads, Raft~\cite{raft} (R-Raft) and Chain Replication (CR)~\cite{chain-replication} (R-CR), and AllConcur~\cite{Poke2016AllConcurLC} (R-AllConcur), a decentralized consensus protocol with consistent local reads. %We build and evaluate these protocols with \projecttitle{} on real hardware. 

To sum up, we make the following contributions:


\begin{itemize}
    \item We present \projecttitle{}, a generic approach for transforming CFT protocols to tolerate Byzantine failures without any modifications to the core of the protocols, e.g., states, message rounds and complexity.
    \item We realize our approach by implementing \projecttitle{}-lib leveraging the advances in modern hardware; we use Trusted Execution Environments (TEEs) to guarantee trust for the executed code and eliminate Byzantine errors. Further, we combine TEEs and direct network I/O (RDMA/DPDK~\cite{rdma, dpdk}) for performance.
    \item We provide proofs of correctness and we show the generality of \projecttitle{} by applying it to four CFT protocols.
    \item Lastly, we evaluate these four protocols against BFT-smart~\cite{bft-smart}, an optimized version of PBFT~\cite{Castro:2002} and Damysus~\cite{10.1145/3492321.3519568}, a transformed \addition{(using TEEs)} version of HotStuff~\cite{DBLP:journals/corr/abs-1803-05069} with $2f+1$ replicas. Our evaluation shows that \projecttitle{} achieves up to $24\times$ and $5.9\times$ better throughput w.r.t. PBFT and Damysus, respectively, while improving scalability---\projecttitle{} requires $2f+1$ replicas, $f$ fewer replicas compared to PBFT ($3f+1$). We further show that \projecttitle{} can offer confidentiality---a security property not provided by traditional BFT protocols---while achieving a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.
\end{itemize}

 \vspace{10pt}

\noindent{\bf {Limitations of \projecttitle{}.}} While \projecttitle{} remains generic, it has been build on top of Intel SGX, which has been abandoned. However,  we believe that this unfortunate event is not restrictive for \projecttitle{}'s adoption. Instead, the state-of-the-art TEEs, such as Intel TDX~\cite{intelTDX} and AMD SEV~\cite{amd-sev}, can support \projecttitle{} out-of-the-box while also facilitate the development of new transformed protocols even more as they come with trusted timer sources~\cite{intelTSC, amdTSC}.

==> intro3.tex <==
\section{Introduction}
\label{sec:introduction}

Replication protocols play the foundational role in designing distributed systems, including distributed storage systems~\cite{10.14778/3007263.3007267, 10.14778/2002938.2002939, zippydb, bankDB, NetflixDB, GEDB, HESSDB}, distributed ledgers~\cite{baasAlibaba, baasAWS, baasAzure, baasIBM, baasOracle}, distributed data analytics systems~\cite{NetflixDB}.  For performance and fault tolerance requirements, distributed systems employ a {\em replication protocol} to maintain a consistent view of the datasets while improving the performance for read-heavy workloads and, more importantly, guaranteeing fault tolerance, {\em i.e.,} reliability and availability in the presence of failures~\cite{zippydb, dynamo, lakshman2009, redis, rocksdb, leveldb, memcached2004, bfthyperledger}.



%These systems employ replication protocols to deal with system failures, e.g., network links, machines, that are present in the cloud infrastructure without violating their correctness. 



%Get to the point!

%As such, the software systems
%need to be constructed in a manner that treats failures as the
%norm rather than the exception.
%\addition{Distributed data stores ub}


%These applications require frequent data store accesses to process user requests that typically present read-heavy access patterns~\cite{246158, 10.14778/3523210.3523213} (REMOVE HERE). To improve user experience, such systems strive to provide fault tolerance without sacrificing performance or consistency~\cite{Herlihy:1990, attiya:1991}.

For handling failures, distributed systems predominately employ Crash Fault Tolerant (CFT) replication protocols~\cite{raft,chain-replication, 10.5555/1855807.1855818, Reed2008AST, 10.5555/800253.807732, lynch:1997, 10.1145/279227.279229, Hermes:2020} to provide consistent replication assuming a {\em fail-stop fault model}, {\em i.e.}, replicas are honest and can only fail by crashing~\cite{delporte}. Unfortunately, CFT protocols are {\em inadequate} for modern untrusted cloud environments, where the underlying cloud infrastructure can be compromised by an adversary, {\em e.g.}, co-located tenants or even a misbehaving cloud operator that may eavesdrop or actively influence the replicas' behavior. In such an untrusted environment, the surface of faults and attacks expands beyond the CFT fail-stop model, ranging from software bugs and configuration errors to malicious attacks~\cite{Gunawi_bugs-in-the-cloud, Shinde2016, hahnel2017high}. CFT protocols are fundamentally incapable of providing consistent replication in the presence of non-benign faults in untrusted cloud environments.


 


%\pramod{why do we need the following text?!} CFT protocols can be either leader-based~\cite{raft,chain-replication, 10.5555/1855807.1855818, Reed2008AST, 10.5555/800253.807732} where a designated node, the leader, drives the protocol execution or decentralized~\cite{lynch:1997, 10.1145/279227.279229, Hermes:2020} where there is no leader and participant nodes (or replicas) propose and execute requests coordinating with each other. We provide a taxonomy of stronly-consistent CFT protocols in $\S$~\ref{sec:background:CFT}.

%However, our growing reliance on online services not only does it require high availability and performance but trustworthy replication too. CFT protocols assume a fail-stop fault model; replicas are honest and can only fail by crashing~\cite{delporte}. However, there is evidence that  the surface of faults and attacks in the third-party untrusted cloud infrastructure has now been expanded beyond the CFT model, ranging from software bugs and configuration errors to malicious attacks~\cite{Gunawi_bugs-in-the-cloud, Shinde2016, hahnel2017high}. Unfortunately, CFT protocols are fundamentally incapable of providing consistent replication in the presence of non-benign faults.


To overcome the limitations of  CFT protocols, Byzantine Fault Tolerant (BFT) protocols~\cite{Lamport:1982} offer important foundations for developing distributed data stores with stronger guarantees in the presence of {\em Byzantine failures}, {\em i.e.}, nodes can fail in arbitrary ways. While BFT protocols can tolerate Byzantine failures, {\em including malicious adversaries}, they are unfortunately {\em not adopted in practice} because of their high-performance and replication resource overheads, and implementation complexity~\cite{visigoth-eurosys}. For instance, BFT protocols require $3f+1$ replicas instead of the $2f+1$ replicas required by CFT protocols for tolerating $f$ faults. BFT protocols also require additional communication rounds (at least three phases instead of two phases in the CFT model); thus incurring high latency and reduced read/write throughput. Lastly, BFT protocols are extremely complex and hard to understand, let alone to implement correctly and optimize~\cite{unsafeZyzzyva}: even intuitive algorithmic optimizations can strongly affect other parts of the protocol~\cite{10.1145/2658994}.

The  “CFT vs. BFT" conundrum creates a fundamental design trade-off between the {\em efficiency of CFT protocols} for practical deployments and the {\em robustness of BFT protocols} for Byzantine settings of modern cloud environments. To strike a balance, our work targets the following research question: {\em How can we design robust and efficient replication protocols for distributed systems hosted in untrusted cloud environments?}

%\myparagraph{Limitations of prior work} Previous research~\cite{minBFT, hybster, DBLP:journals/corr/LiuLKA16a, A2M, 10.1145/2168836.2168866} made an effort to optimize BFT protocols by reducing the number of replicas required using trusted hardware. Specifically, they use trusted modules along with the protocol's ``traditional'' (untrusted/Byzantine) counterpart to prevent Byzantine processes from making conflicting statements for the same request (equivocation). Unfortunately, as before, all of these efforts require programmers to understand, transform and optimize such complex protocols; a task as challenging as it is error-prone. Consequently, BFT protocols are still not widely adopted by cloud services~\cite{bft-time-is-now, 10.1145/1711475.1711494} that, instead, sacrifice security and rely on CFT protocols to handle failures~\cite{Hunt:2010, etcd, zippy, redis, rafthyperledger}.


%Unfortunately, traditional BFT protocols present severe limitations that impede their adoption in modern, high-end distributed systems ($\S$~\ref{sec:background:CFT}). First, classical BFT protocols are limited in performance and scalability: they incur high message complexity and mulitple rounds~\cite{} deploying at least $3f+1$ nodes to tolerate up to $f$ Byzantine nodes. Secondly, BFT replication is complex, introducing burdens to developers \dimitra{say something more here to strengthen this}.



%\noindent{\underline{\#1: Performance and scalability.}} BFT protocols are slow due to high message complexity (typically, $O(n^2)$) and multiple protocol rounds while they require at least $3f+1$ nodes to tolerate up to $f$ Byzantine nodes which severely limits scalability. In contrast, widely adopted CFT protocols~\cite{raft, Reed2008AST, primary-backup, engraft} comprise two rounds and $O(n)$ message complexity with $2f+1$ replicas.


%\noindent{\underline{\#2: Complexity and adoption.}} BFT protocols are complex, introducing burdens to developers. Even if system designers wish to use a state-of-the-art BFT protocol, optimizing it for the specific application settings (e.g., network bandwidth,  number of clients and replicas, cryptographic libraries, etc.) can be complicated. Guerraoui et al.~\cite{10.1145/2658994} found that most protocol implementations consist of thousands of lines of code, e.g., PBFT~\cite{Castro:2002} and Zyzzyva~\cite{10.1145/1658357.1658358}. Even trivial changes or intuitive optimizations can be extremely hard and might affect other parts of the protocol (e.g., view-change in Zyzzyva).



%%%All the above in combination with the difficulty of testing distributed protocols~\cite{Chandra2007PaxosML} require great effort for designing and optimizing such protocols. Consequently, BFT protocols are still not widely adopted by cloud services~\cite{bft-time-is-now, 10.1145/1711475.1711494} that, instead, rely on CFT protocols to handle failures~\cite{Hunt:2010,etcd, zippy, 51, redis}.



%The only complete proof of a BFT protocol we knew of is that of PBFT and it involves 35 pages (even without using any formal language).1 This difficulty, together with the impossibility of exhaustively testing distributed protocols [8] would rather plead for never changing a protocol that was tested and proven correct, e.g., PBFT.

%%%%% Previous works~\cite{minBFT, hybster, DBLP:journals/corr/LiuLKA16a, A2M, 10.1145/2168836.2168866} aim at optimizing BFT protocols and mostly focus on reducing the number of replicas required. They use trusted modules along with the protocol's ``traditional'' (untrusted) counterpart to prevent Byzantine processes from making conflicting statements for the same request (equivocation). As before, all of these efforts require programmers to understand, transform and optimize these complex protocols; a task that is quite challenging.




%{\em ``The solution lies within the problem!"}---our work 

Our work leverages modern cloud hardware for transforming existing CFT protocols for Byzantine settings in untrusted cloud environments. Specifically, our transformation underpins the robustness and efficiency axes.
For {\em robustness}, we leverage trusted hardware available as part of confidential cloud computing to harden the security properties of CFT protocols~\cite{intel-sgx, keystone_eurosys, amd-sev, intelTDX}. In particular, we leverage trusted execution environments (TEEs) to provide two key properties for successfully transforming a CFT protocol to operate in Byzantine settings, as identified by Clements et al.~\cite{clement2012}: (a) transferable authentication, {\em i.e.}, the ability to establish trust in nodes in distributed settings by designing a remote attestation protocol, and (b) non-equivocation, i.e., once the trust is established in a node via the remote attestation protocol, the node follows the CFT replication protocol faithfully, and therefore, it cannot send conflicting statements to other nodes. %to reach agreement in the presence of Byzantine faults in the asynchronous communication model.

For {\em efficiency}, we leverage the modern networking hardware, such as RDMA/DPDK for kernel bypass, to design a highly optimized communication protocol for replicating the state across nodes in distributed settings~\cite{rdma, dpdk, erpc}, while overcoming the I/O bottlenecks in trusted computing~\cite{rkt-io}.


%Specifically, we leverage \emph{(1)} trusted hardware to harden the properties of CFT protocols building a transformation of CFT protocols for Byzantine settings and \emph{(2)} modern networking (direct I/O) for efficiency. In addition, we show that our transformation can \emph{transparently} offer confidentiality to applications when they need it~\cite{ciad} ($\S$~\ref{sec:motivation}), an extra property not offered by traditional BFT, without sacrificing performance. More importantly, we give system designers the opportunity to build protocols that tolerate Byzantine faults without having to become BFT experts.


\myparagraph{Our proposal: \projecttitle{}} 
\projecttitle{} leverages TEEs along with direct I/O to resolve the tension between security and performance by building an efficient and practical transformation of unmodified CFT replication protocols for Byzantine settings. \projecttitle{} achieve this by implementing a distributed Trusted Computing Base (TCB) that shields the replication protocol execution and {\em extends} the security properties offered by a single TEE (whose security properties are only effective in a single-node setup) to a distributed setting of TEEs. Our design is comprised of a transferable authentication phase ($\S$~\ref{sec:attestation}) for distributed trust establishment, a high-performant network stack for secure communication over the untrusted network ($\S$~\ref{subsec:networkin}) and a memory-efficient KV store ($\S$~\ref{subsec:KV}). 

% implementing a distributed Trusted Computing Base (TCB) that shields communication .. %..that transforms unmodified CFT protocols for Byzantine settings. We explore and realize the potential of Trusted Execution Environments (TEEs) to build 

%We explore and realize the potential of Trusted Execution Environments (TEEs) to build an efficient and practical transformation, a ``\projecttitle{}'', of a CFT protocol for Byzantine settings.  If used naively, however, TEEs incur great overheads~\cite{10.5555/1924943.1924946}. In this paper, we show how we can mitigate the performance impact of using TEEs by adopting direct network I/O. As a result, our approach offers BFT while providing {\em better performance (and security, i.e., confidentiality) than conventional BFT protocols} and reaping {\em all the benefits of CFT protocols} (fewer nodes, easier implementation, simplicity).

%To sum up, this paper poses the following question: \emph{Can we leverage (and how) the advances in trusted computing and  networking, like Trusted Execution Environments (TEEs) and direct I/O, to harden the properties of CFT protocols to (1) target a weaker fault model (i.e., Byzantine faults) while (2) offering performance and scalability?}

%Our answer is \projecttitle{}, an approach to transform a CFT protocol to handle Byzantine faults. We materialize the \projecttitle{} approach as a generic library, \projecttitle{}-lib, that prevents equivocation and guarantees authentication for the network. Our key insight is the use of modern hardware to achieve both BFT and performance---two often contradictory goals; we use TEEs for trust and direct network I/O for performance.

We materialise \projecttitle{} approach as a generic library, \projecttitle{}-lib ($\S$~\ref{sec:recipe-implementation}), on top of Intel SGX and the \scone{} framework~\cite{arnautov2016scone}. We carefully build \projecttitle{}'s high-performance network stack for TEEs, extending eRPC~\cite{erpc} to enable direct I/O, essentially DMA operations, within the protected TEE domain while shielding the exchanged messages to maintain authenticity and non-equivocation accross the network. Lastly, our lock-free KV store is designed to optimize for the limited trusted area in TEEs~\cite{speicher-fast, shieldstore}.% on top of folly library~\cite{folly}.

%Our , built on top of TEEs and direct network I/O, follows an established RPC-API, e.g., RDMA programming paradigm~\cite{rdma}, allowing system designers to seamlessly transform a CFT protocol for Byzantine settings. We implement \projecttitle{}-lib on top of Intel SGX~\cite{intel-sgx} and \scone{}. In addition, we extend eRPC~\cite{erpc} (on top of DPDK~\cite{dpdk}) and we build a shielded high-performant RPC library, carefully designed for TEEs, that preserves non-equivocation and authentication in the untrusted network.


Our evaluation assesses \projecttitle{}'s generality and efficiency. Specifically, to show the generality of our approach, we apply and evaluate \projecttitle{} on real hardware with four well-known CFT protocols (from now on, an `R-' prefix stands for the transformed protocol); a decentralized (leaderless) linearizable multi-writer multi-reader protocol (ABD)~\cite{lynch:1997} (R-ABD), two leader-based protocols with linearizable reads, Raft~\cite{raft} (R-Raft) and Chain Replication (CR)~\cite{chain-replication} (R-CR), and AllConcur~\cite{Poke2016AllConcurLC} (R-AllConcur), a decentralized consensus protocol with consistent local reads. To evaluate performance, we compare \projecttitle{} protocols with two competitive BFT replication protocols, BFT-smart~\cite{bft-smart}, whose specific implementation has been adopted in industry~\cite{bftsmarthyperledger} and Damysus~\cite{10.1145/3492321.3519568} a state-of-the-art BFT replication protocol.  Our evaluation shows that \projecttitle{} achieves up to $24\times$ and $5.9\times$ better throughput w.r.t. PBFT and Damysus, respectively, while improving scalability---\projecttitle{} requires $2f+1$ replicas, $f$ fewer replicas compared to PBFT ($3f+1$). We further show that \projecttitle{} can offer confidentiality---a security property not provided by traditional BFT protocols---while achieving a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.

\myparagraph{Artifact} \projecttitle{} is available as an open-source project.%: \url{https://anonymous.4open.science/r/secure_replication-907F/}.


%build on top of Intel SGX. Our \projecttitle{} up to $24\times$ and $5.9\times$ better throughput w.r.t. BFT-smart and Damysus.

\if 0
\myparagraph{Contributions} Overall, we make the following contributions:


\begin{itemize}[leftmargin=*]
    \item {\bf Hardware-assisted transformation of CFT protocols:} We present \projecttitle{}, a generic approach for transforming CFT protocols to tolerate Byzantine failures without any modifications to the core of the protocols, e.g., states, message rounds, and complexity. We realize our approach by implementing \projecttitle{}-lib leveraging the advances in modern hardware; we use trusted hardware to guarantee transferrable authentication and non-equivocation for thwarting Byzantine errors. Further, we combine trusted hardware with direct network I/O (RDMA/DPDK~\cite{rdma, dpdk}) for performance.

    \item {\bf Generic \projecttitle{} APIs:} We propose generic \projecttitle{} APIs to transform the existing codebase of CFT protocols for Byzantine settings. Using \projecttitle{} APIs, we have successfully
transformed a range of leader-/leaderless-based CFT protocols enforcing different (total order/per-key) ordering semantics.  We further show that \projecttitle{} can offer confidentiality---a security property not provided by traditional BFT protocols.

    
    \item {\bf Formal correctness analysis:}  We provide a correctness analysis for the safety and liveness properties of our
transformation of CFT protocols operating in Byzantine settings. % We provide a formal analysis showing the correctness and 
    \item {\bf \projecttitle{} in action:} We present an extensive evaluation of \projecttitle{} by applying it to four CFT protocols: Chain Replication, Raft, ABD, and AllConcur. We evaluate these four protocols against the state-of-the-art BFT protocol implementations and show that \projecttitle{} achieves up to $24\times$ and $5.9\times$ better throughput.
    
  %  BFT-smart~\cite{bft-smart}, an optimized version of PBFT~\cite{Castro:2002} and Damysus~\cite{10.1145/3492321.3519568}, an optimized version of HotStuff~\cite{DBLP:journals/corr/abs-1803-05069}. Our evaluation shows that \projecttitle{} achieves up to $24\times$ and $5.9\times$ better throughput w.r.t. PBFT and Damysus, respectively, while improving scalability---\projecttitle{} requires $2f+1$ replicas, $f$ fewer replicas compared to PBFT ($3f+1$). We further show that \projecttitle{} can offer confidentiality---a security property not provided by traditional BFT protocols---while achieving a speedup of $7\times$---$13\times$ w.r.t. PBFT and up to $4.9\times$ w.r.t. Damysus.
\end{itemize}

\fi 
%  \vspace{10pt}

% \noindent{\bf {Limitations of \projecttitle{}.}} While \projecttitle{} remains generic, it has been build on top of Intel SGX, which has been abandoned. However,  we believe that this unfortunate event is not restrictive for \projecttitle{}'s adoption. Instead, the state-of-the-art TEEs, such as Intel TDX~\cite{intelTDX} and AMD SEV~\cite{amd-sev}, can support \projecttitle{} out-of-the-box. These TEEs can also facilitate the development and improve the performance of new transformed protocols as they overcome some core architectural limitations of Intel SGX ($\S$~\ref{sub:background:TEE}). Particularly, they come with larger trusted memory~\cite{intelTDX2} and trusted timer sources~\cite{intelTSC, amdTSC}.

==> overview.tex <==
\section{Model and Preliminary Definitions}
\label{sec:design}

\subsection{The CFT Vs. BFT Conundrum}
\label{sec:background:CFT}




\myparagraph{CFT protocols}
CFT protocols assume that the infrastructure is trusted. These protocols tolerate only benign faults; replicas can fail by stopping or by omitting some steps~\cite{delporte}. As such, while having low overheads, they are not suitable for modern applications deployed in third-party untrusted cloud infrastructure~\cite{10.1145/3190508.3190538}. In this paper, we evaluate protocols that enforce either sequential consistency~\cite{1675439} or linearizability~\cite{Herlihy:1990}, also referred to as \emph{strongly-consistent} replication protocols.




We can broadly split strongly-consistent CFT protocols into two categories (see Table~\ref{tab:categories} for the taxonomy):  \emph{(i)} leader-based protocols (e.g., Raft~\cite{raft}, Chain Replication (CR)~\cite{chain-replication}), where a node, designated as a leader, drives the protocol execution and \emph{(ii)} decentralized protocols (e.g., ABD~\cite{lynch:1997},  AllConcur~\cite{Poke2016AllConcurLC}), where there is no leader and all nodes can propose and execute requests. 

We further divide them based on their ordering semantics. First, protocols with total ordering, where the protocols create a total order of all writes across all keys and apply them in that order. Second, protocols with per-key ordering semantics where the protocol enforces the total order of writes on a per-key basis. The evaluation of \projecttitle{} ($\S$~\ref{sec:eval}) relies on this taxonomy to systematically study its protocols' performance, as these two dimensions significantly impact the performance of the CFT protocols~\cite{f04eb9b864204bab958e72055062748c}. %By implementing and evaluating one protocol of each category with \projecttitle{} ($\S$¬\ref{sec:eval}) not only do we study the performance characteristics of protocols of the entire category but we further show the generality of our approach.

%These characteristics lead to a taxonomy of four categories summarized in Table~\ref{tab:categories}.

%We chose these two characteristics to categorise the protocols because they have been proven to impact performance the most~\cite{f04eb9b864204bab958e72055062748c}. Briefly, protocols that offer total order might introduce scalability bottlenecks due to coordination costs whereas leader-based protocols can also limit scalability as a single node, i.e., the leader, is the point of serialization. On the other hand, leader-less or per-key ordered protocols can support more parallelism but they might require distributed coordination, and as a result, more resources (e.g., network, locks) to serialize writes.



\begin{table}[t]
\small
%\fontsize{9}{10}\selectfont 

\fontsize{7}{10}\selectfont 
\begin{center}
\begin{tabular}{ | p{2.8cm} | p{3.6cm} | p{3.6cm} | }
\rowcolor{gray!25}
 \hline
 & \bf{Leader-based} & \bf{Leader-less} \\ \hline
     \multirow{2}{*}{\bf{Total order}}  & {\bf{Raft}}~\cite{raft}, ZAB~\cite{Reed2008AST},            & {\bf{AllConcur}}~\cite{Poke2016AllConcurLC}, \\ 
 & Multi-Paxos~\cite{10.1145/2673577} & Derecho~\cite{derecho}                         \\ \hline
 
    \multirow{2}{*}{\bf{Per-key order}}  & {\bf{CR}}~\cite{chain-replication}, CRAQ~\cite{10.5555/1855807.1855818},& {\bf{ABD}}~\cite{lynch:1997}, CP~\cite{10.1145/279227.279229},  \\ 
      & PB~\cite{primary-backup}, CHT~\cite{cht}  &  Hermes~\cite{Hermes:2020} \\
\hline
\end{tabular}
\end{center}
%\vspace{-10pt}
\caption{CFT protocols taxonomy. Using \projecttitle{}, we transform one protocol (shown in bold) of each category.} \label{tab:categories}
\vspace{-2pt}
\end{table}

\myparagraph{BFT protocols} 
In contrast to CFT protocols, BFT protocols assume very little about the nodes and the network; faulty nodes may behave arbitrarily while the network is unreliable. To tolerate $f$ arbitrarily faulty processes that may \emph{equivocate} (i.e., make conflicting statements for the same request to different replicas), BFT protocols add $f$ extra replicas to their system model requiring at least $3f+1$ replicas for safety. As such, BFT protocols exhibit worse scalability compared to CFT protocols (which only require at most $2f+1$ replicas).

BFT protocols are limited in performance, too. They incur high message complexity ($O(f^2)$)~\cite{10.1145/2168836.2168866, Castro:2002, minBFT}, multiple protocol rounds~\cite{DBLP:journals/corr/LiuLKA16a, 10.1145/2168836.2168866, Castro:2002, DBLP:journals/corr/abs-1803-05069, yandamuri} and complex recovery ($O(f^2)$ in view-change)~\cite{DBLP:journals/corr/LiuLKA16a, Castro:2002, minBFT, 10.1145/2168836.2168866}. As an example of this, PBFT~\cite{Castro:2002}, a well-known BFT protocol, requires at least $3f+1$ nodes, executes three broadcast rounds, and incurs $O(n^2)$ message complexity. %HotStuff~\cite{DBLP:journals/corr/abs-1803-05069}, on the other hand, simplifies message complexity ($O(f)$) at the cost of extra communication steps: it requires 5 phases (\texttt{pre-prepare}, \texttt{prepare} and \texttt{commit} along with two complementary phases, \texttt{new-phase} and \texttt{decide}) at each round. 

%In addition, BFT protocols require at least $3f+1$ nodes to tolerate up to $f$ Byzantine nodes which severely limits scalability. In contrast, widely adopted CFT protocols~\cite{raft, Reed2008AST, primary-backup, engraft} comprise two rounds and $O(n)$ message complexity with $2f+1$ replicas.


Thirdly, BFT protocols are complex, introducing burdens to developers. Guerraoui et al.~\cite{10.1145/2658994} found that most protocol implementations consist of thousands of lines of (non-trivial) code, e.g., PBFT~\cite{Castro:2002} and Zyzzyva~\cite{10.1145/1658357.1658358}. Even if system designers wish to use a state-of-the-art BFT protocol, optimizing it for the specific application settings (e.g., network bandwidth,  number of clients and replicas, cryptographic libraries, etc.) is a rather complicated task.  Even trivial changes or intuitive optimizations can be extremely hard and might affect other parts of the protocol (e.g., view-change in Zyzzyva).





\subsection{Transformation Requirements}
\label{subsec:req}

The basic requirements for transforming a CFT protocol for Byzantine environments are established in a theoretical result published by Clement et al. in PODC 2012~\cite{clement2012}. This seminal paper shows that non-equivocation and transferable authentication are necessary to go from $3f+1$ to $2f+1$ replicas for a reliable broadcast in Byzantine settings. Our work shows that not only can this lower bound be achieved in practice, we can do so while providing high performance by leveraging modern hardware in a cloud environment. Next we discuss how \projecttitle{} satisfies these two fundamental requirements, while $\S$~\ref{sec:motivation} elaborates on how to design \em{practical} and \em{efficient} protocols that meet these requirements.


\noindent{}{\bf{\underline{Property 1:}}} The transferable authentication property refers to the authenticity of a received message, requiring that a replica must be able to verify that the supposed sender indeed had sent the message. The authentication is transferable if the original sender can be verified even for forwarded messages. Formally, a message $m$ received by a correct process $P_j$ from $P_i$ is verifiable by any other correct process $P_k$. That is, given an authentication proof $\sigma_i$: 
\[
\forall P_k : \text{Verify}(m, \sigma_i, P_i) \Rightarrow \text{Accept}(m, P_k)
\]

\noindent{}{\bf{Mechanism 1:}} \projecttitle{} employs cryptographic primitives and an attestation protocol. The cryptographic primitives ensure that nodes can generate and validate authenticated messages while \projecttitle{}'s attestation protocol ($\S$~\ref{sec:attestation}) ensures that only trusted replicas access the cryptographic keys and execute the protocol.

\noindent{}{\bf{\underline{Property 2:}}} The non-equivocation property guarantees that replicas cannot \emph{accept} conflicting statements for the same request. That implies that \projecttitle{} must detect attacks where adversaries try to compromise the protocol by sending invalid requests or by re-sending valid but stale requests (\emph{replay attacks}). Formally, a Byzantine node $P_i$ cannot produce two conflicting statements $m$ and $m'$ for the same operation to different correct replicas $P_j$ and $P_k$: \[
\forall P_j, P_k, \quad (P_i \xrightarrow{} P_j : m) \wedge (P_i \xrightarrow{} P_k : m') \Rightarrow m = m'
\]

\noindent{}{\bf{Mechanism 2:}} \projecttitle{} prevents equivocation by materializing a distributed TCB that shields the protocol's (distributed) execution as well as shielding the network communication based on an authenticated message format ($\S$~\ref{sec:normal_operation}). 


==> recipe_design-old.tex <==
\section{\projecttitle{}}
%\subsection{}
\label{sec:design}


%\dimitra{reminder: ONE paragraph -> one point, MANY points under the same par -> subparag}


%\dimitra{do an OVERVIEW as a subsection that serves two things: 1) the link between 4 \& 5 and 2) give the intuition}

\subsection{Overview}
%\projecttitle{} provides a general transformation of CFT protocols to target performance under Byzantine settings. 
\dimitra{SOS FIX ME EVERYWHERE: 5.1, 5.3 and 5.5.!}
Figure~\ref{fig:overview} shows the overview of the \projecttitle{} system.  We base our design on a distributed setting of TEEs that implement a (distributed) trusted computing base (TCB) and shield the execution of unmodified CFT protocols against Byzantine failures. \projecttitle{}'s TCB contains the protocol's code along with some metadata which, among others, include the configuration, the view id, the status of the replica, etc. (Table~\ref{tab:meta}). Replicas receive secrets (e.g., encryption keys) and configuration in a secure manner at initialization ($\S$~\ref{subsec:attestation}).

Further, \projecttitle{} builds a networking library to achieve low-latency communication between replicas ($\S$~\ref{subsec:networkin}). Our library shields the communication against Byzantine actors by guaranteeing the non-equivocation and transferable authentication across the network. \projecttitle{} guarantees both properties by layering the non-equivocation and authentication layers on top of the direct I/O library. We present an overview of the properties and the mechanism ($\S$~\ref{subsec:req}), the detailed description ($\S$~\ref{subsec:networkin}), and the correctness analysis ($\S$~\ref{sec:theory}).


%layer ensures that replicas will not miss any past messages. The authentication layer ensures integrity and authenticity for the network messages; replicas can .

%which shield the network stack against Byzantine errors. 

Lastly, \projecttitle{} builds a KV store which increases the trust to individual nodes allowing for local reads ($\S$~\ref{subsec:KV}). In reality, our KV store achieves two goals; first we guarantee trust to individual replicas to serve reads locally and secondly we limit the TCB size optimizing the enclave memory usage. As shown in Figure~\ref{fig:overview}, \projecttitle{} keeps bulk data (values) in the host memory and stores only minimal data (keys + metadata) in the enclave area. The metadata, i.g., hash of the value, timestamps, etc. are kept along with keys in the TEE for verifying the integrity of the unprotected values.

\subsection{Requirements for Transformation: An Overview}
\label{subsec:req}
We next discuss how \projecttitle{} satisfies the requirements for the tansformation~\cite{clement2012}.

%Prior work~\cite{clement2012} proves theoretically that non-equivocation
%and transferable authentication are the lower bounds to replace the bound $f<n/3$ by $f<n/2$ (where $f$ is the number of faulty replicas and $n$ the total number of replicas) for a reliable broadcast in Byzantine settings.  

\noindent{}{\bf{\underline{Property 1:}}} The transferable authentication property refers to the authenticity of a received message, requiring that a replica must be able to verify that the supposed sender indeed had sent the message. The authentication is transferable if the sender can be verified even if the message is forwarded by a replica other than the original sender. 

\noindent{}{\bf{Mechanism 1:}} \projecttitle{}'s authentication layer relies on cryptographic attestation primitives to ensure the property. We calculate the hash of the message's payload which we encrypt with a secret key along with some metadata. Only trusted nodes that have the key can decrypt the message, which is ensured by remote attestation~\cite{Parno2010}.% \pramod{cite remote attestation paper}

\noindent{}{\bf{\underline{Property 2:}}} The non-equivocation property guarantees that replicas cannot \emph{accept} conflicting statements for the same request. That implies that \projecttitle{} must detect attacks where adversaries try to compromise the protocol by sending invalid requests or by re-sending valid, but stale, requests (\emph{replay attacks}). 

\noindent{}{\bf{Mechanism 2:}} \projecttitle{}'s non-equivocation layer assigns sequence ids to network messages to guarantee that replicas cannot miss past messages (or double-execute them). In addition, the authentication layer guarantees that invalid requests that are not signed with the secret key are detected.






\subsection{Normal Operation: DIMITRA: NEEDS CHANGE GIVEN THE FIGURE}
\label{sec:normal_operation}

\begin{figure*}
    \begin{center}
        %\includegraphics[width=0.8\textwidth]{figs/recipe_overview.pdf}
        %\includegraphics[width=0.38\textwidth]{figs/raft_recipe.pdf}
        \includegraphics[width=\textwidth]{figs/recipe_protocol_overview3.pdf}
        %\vspace{-4pt}
        \caption{Example of R-Raft execution.}
        \label{fig:raft_example}
        %\vspace{-24pt}
    \end{center}
\end{figure*}



\if 0
\dimitra{\begin{itemize}
    \item clients are running requests through a \texttt{PUT}/\texttt{GET} API. 
    \item describe the clients' requirements (message format, ids, term/view/leader identifier etc.)
    \item a \projecttitle{}'s coordinator receives the request: 
    \begin{itemize}
        \item verify integrity (and/or confidentiality)
        \item execute the underlying protocol implementation (tell how put/get operations are executed, when the application is considered committed, tell about the uncommitted queues, etc.). 
        \item update metadata (client table, commit idx, last seen message idx, etc.) and app state
        \item cleanup history if required
        \item reply to the client (reply format, etc.)
    \end{itemize}
\end{itemize}
}
\fi

\if 0
\begin{itemize}
    \item the configuration (i.e., the encryption keys for network and application state and the IPs of the nodes along with their replica number).
%    \item the metadata index for networking (i.e., a node stores for each replica the latest processed message index and a queue with the on-hold message identifiers).
    \item the clients table which stores the most recent operation seen from a client (identified by an id).
    \item the term and the leader identifiers in the case of a leader-based underlying protocol.
    \item the operation status of the replica (i.e., \texttt{Normal}, \texttt{Recovering}, \texttt{View\_change}).
    \item the leases table (i.e., access leases for local reads and/or other nodes' leases).
    \item an index store for the application's state that holds metadata for the integrity and/security checks.
\end{itemize}
\fi




\begin{table}[t]
%\small
\fontsize{9}{10}\selectfont 

%\fontsize{8}{10}\selectfont 

\begin{center}
\begin{tabular}{ |l|c| }
 \hline
 \multirow{1}{*}{The configuration} & Encryption keys, IPs, etc.\\ \hline
 \multirow{1}{*}{The clients table} & \multirow{1}{*}{Last req id seen from a client.}\\ \hline
 The view (term) & \multirow{2}{*}{For leader-based CFT protocols.}\\ and leader id & \\ \hline
 Replicas operation &  \texttt{Normal}, \texttt{Recovering}, \texttt{ViewChange}.\\ \hline
 %\multirow{1}{*}{The leases table} & \multirow{1}{*}{Access leases for local reads and/or other nodes' leases.} \\ 
 \multirow{2}{*}{The (hybrid) KV store} & Stores the metadata in the TEE\\
 &  and bulk data in host memory.\\ \hline
\end{tabular}
\end{center}
%\vspace{-10pt}
\caption{\projecttitle{}'s metadata in the TEE.}\label{tab:meta}
%\vspace{-18pt}
\end{table}


Clients in \projecttitle{} execute requests through a \texttt{PUT}/\texttt{GET} API by sending the request to the coordinator node. Figure~\ref{fig:raft_example} shows as an example a \projecttitle{} implementation of Raft (R-Raft). The leader initializes the underlying CFT protocol to execute the request \circled{2}---\circled{3a},\circled{3b}---\circled{4}---\circled{5} and, upon completion, replies to clients \circled{6a}, \circled{6b}. Next we discuss the \projecttitle{} abstraction under Normal operation. %\manos{some repetition with the system model (\$3) now}

 %In leaderless protocols, coordinator nodes are selected randomly. In leader-based protocols, all non-leader replicas deny to process requests and reply back to clients with their view of the current active leader. The client then can forward the request to the active leader.


%\begin{itemize}[noitemsep]
  %\setlength\itemsep{10em}
    \noindent{}{\bf{\underline{\#1}}:} Clients send to the coordinator their request of the form $<(metadata, req\_data)$, $h_{c}>_{\sigma_{c}}$. The req\_data is the request's associated data and the metadata might include among others the client id, the leader's and term's ids (known to the client), and the request id. The request is sent over the network along with the message's calculated signed hash $h_{c}$. We use the symbol $\sigma_{c}$ to denote that the message is signed with a key $c$.
    %Clients send to a node (from now on the request's \emph{coordinator node} or leader), their preferred request that is of the form <$\texttt{CLIENT\_REQ(cid, lid, tid, rid, rdata)}$, $h_{c}$> where \texttt{cid} is the client id, \texttt{lid} and \texttt{tid} is the leader's and term's ids known to the client, \texttt{rid} is the request id which gets monotonically incremented per client and \texttt{rdata} is the serialized request with its arguments. The request is sent over the network along with the message's calculated signed hash $h_{c}$.
    
    \noindent{}{\bf{\underline{\#2}}:} Nodes receive and process a request as long as they are authorized to do so. Essentially, requests that have a wrong view of the term and the leader or have already processed (their id is known to the coordinator node) are dropped.
%    \dimitra{MAKE THE PAR shorter in all paper -> make it as substeps}
    
    \noindent{}{\bf{\underline{\#3}}:} Upon the reception of a client's request: 
    
    {\bf{\#3.1}} The coordinator node verifies the integrity and authenticity of the message using \projecttitle{}'s authentication layer. The node also verifies the metadata, e.g., the message is not valid if the term and the leader (if any) known to the client are not correct. The coordinator updates the client table with the latest processed request for each client. 
    
    {\bf{\#3.2}} Next, the coordinator initializes the protocol for that request. In our example, the Raft leader receives the request \circled{2} and passes through Raft's replication phase by multi-casting the \texttt{PUT} request to the majority \circled{3a}---\circled{3b}. Once the majority acknowledges the request (red arrows), the leader initiates the second round of the protocol instructing the majority to commit the update. The execution returns back to the client after the majority acks the commit \circled{5}---\circled{6a}. 
    
    {\bf{\#3.3}} The messages exchanged between replicas are of the form $<(metadata, req\_data)$, $h_{r}>_{\sigma_{cq}}$. The metadata include a per-request unique tuple which contains the view, the communication channel id and a sequencer id for that channel ($<$$view, cq, cnt$$>$). The sequencer id is increased monotonically for every new request sent over the $cq$ (non-equivocation).
    %\dimitra{here: explain the counter}
    %The messages $m$ that are sent between replicas are of the form $<\texttt{CFT\_REQ(cid, lid, tid, rid, rdata), <view, cq, cnt>}$, $h_{m}>_{\sigma_{c}}$. \dimitra{here: explain the counter}
    
    \noindent{}{\bf{\underline{\#4}}:} When a replica receives a message from another replica:
    
    {\bf{\#4.1}} It verifies validity and integrity of the message (authentication-layer). Only replicas in Normal operation mode are authorized to execute the protocol---if the replica's state differs, it might refuse to process the request.% (e.g, Recovering-state replicas do not execute the read path).
    
    {\bf{\#4.2}} The replica verifies the message counter ($msg\_cnt$) through the non-equivocation layer to see if it is consistent with its local counter ($cnt_{cq}$). If the current $msg\_cnt$ equals ($cnt_{cq}$+$1$), the replica executes the request immediately, increases the $commit_{idx}$ and acknowledges to the sender node. The replica also updates the client table. In case the message counter refers to a ``future'' message ($msg\_cnt$ $>$ $cnt_{cq}$+$1$), the replica might queue the request in the protected area. Periodically, \projecttitle{} replicas apply the queued requests that are eligible for execution and notify coordinators accordingly.
    
    \noindent{}{\bf{\underline{\#5}}:} After the protocol's execution for a request, the coordinator marks the request as committed and notifies the client (In our example \circled{6a} and \circled{6b}).
    %\noindent{}{\bf{\underline{\#5}}:} A request coordinator after the protocol's execution for that request updates the state of the request as committed and notifies the client (In our example \circled{6a} and \circled{6b}.).
    
    \noindent{}{\bf{\underline{\#6}}:} Replicas, if required, rely on timeouts and heartbeat messages to verify they are part of the configuration. %In case of untrusted environments, \projecttitle{} models timeouts with trusted leases for TEEs~\cite{t-lease}.
%\end{itemize}





\subsection{View Change}
\if 0
\dimitra{\begin{itemize}
    \item view change is ''leader election`` for us!
    \item Describe how recipe identifies leader failures
    \item Leader election depends on the specific protocol but you must say here how you ensure at most one leader at a time
\end{itemize}
}
\fi

While decentralized protocols remain always available as long as a majority of nodes is part of the membership, the leader-based protocols do not make any progress if the leader goes down. To remain available after the leader crashes, the followers need to closely monitor the leader (e.g., heartbeat messages in inactive periods) and, in case it is unreachable, to \emph{elect} a new one---in PBFT parlance to do a \emph{view change}.

%Usually, the leader sends requests which also notify followers about the leader's activity. However, due to inactivity, the leader might remain idle and in this case it will send pings. 

%The follower nodes rely on timeouts to identify leader failures. Specifically, if a timeout expires without communication (and, probably, after some retries), the replicas need to carry out a leader election protocol to switch to a new leader---similarly, as a view change to switch to a new primary in PBFT. 

\projecttitle{} assigns a leader with a term and the node identifier. The term identifier can be seen as an \emph{epoch}, a monotonically increased number that uniquely identifies the current view of the system. To continue serving requests after a leader election, all replicas of the membership need to confirm the new leader along with the new term. Since a leader needs to be acknowledged by the majority of the nodes to operate, it follows that the latest term will survive in at least one node, which ensures the monotonic increments of the term.

\myparagraph{Correctness} The correctness condition for leader elections is that every committed operation must survive into the new leader election in the order selected for it at the time it was executed. \projecttitle{} does not make further assumptions for leader election, we guarantee that the replicas are trusted ($\S$~\ref{sec:theory}). Protocols can rely on their election algorithms. %Additionally, if the client receives no reply to a request, it resents the request; this way all clients eventually will learn about the new elected leader, and also prompts the new leader/primary to send it the reply.

\myparagraph{Failure detection} Some CFT protocols~\cite{raft, chain-replication} often require a trusted timer source to detect failures. We build \projecttitle{} on top of Intel SGX that is no longer supporting secure timers~\cite{monotoniccounterssgx, sgxtrustedtime}. The OS-timers and software-based implementations of a clock cannot be trusted. %Similarly, any software-based implementations or simulations of a clock within the TEE can be compromised by a Byzantine OS.%---for example, the OS can continuously schedules out the timer thread.\\
Unfortunately, the lack of a trusted timer complicates failure detection for protocols that primarily rely on accurate time-outs---for example, leader election in Raft. \projecttitle{} builds on top of \scone{} that implements a trusted lease mechanism~\cite{t-lease}. Our mechanism supports all the  properties of classical leases~\cite{10.1145/74850.74870} in untrusted environments that is the building block for trusted timeouts, failure detectors~\cite{222603}, leader election~\cite{815321}, etc.

While \projecttitle{}'s overcomes this problem, we believe that this is no longer a real limitation as the state-of-the-art TEEs~\cite{intelTDX, amd-sev} offer trusted timer sources~\cite{intelTSC, amdTSC}. %\projecttitle{}'s lease mechanism supports all the properties of classical leases~\cite{10.1145/74850.74870} while it offers accuracy, performance and correctness in untrusted environments. The lease duration of the holder is always a superset of the granter under the presence of a powerful attacker that can manipulate the clocks, the cpu frequency, etc.
%We argue that this is no longer a limitation as the state-of-the-art TEEs~\cite{intelTDX, amd-sev} offer trusted timer sources~\cite{intelTSC, amdTSC}.


\subsection{Recovery}

As nodes fail, new or recovered nodes need to be added to continue operating at peak performance. To add a new node, the membership needs to be reliably updated, following that all other live replicas are notified of the new node’s
intention to join the replica group. Once all the replicas acknowledge this notification, the new node starts operating as a shadow replica that participates as a follower for  the writes but does not serve any client requests. Additionally, it might read chunks from other replicas to fetch
the latest state and reconstruct the application state similarly to~\cite{10.1145/2815400.2815425, 10.1145/2043556.2043560}. Overall a new joining node follows the next steps:

%\begin{itemize}
   \noindent{}{\bf{\underline{\#1}}:} A recovering node needs first to be attested before any secrets and membership information are shared. Particularly, upon a node recovery or join, before the control passes to the CFT protocol, the node sends a join request to a designated node notifying it about its willingness to join the cluster. %\footnote{While we were implementing \projecttitle{}, we assumed static IP addresses where nodes are listening for join requests. However, this is not a restriction. The developers can implement there own membership management service.}
   
   \noindent{}{\bf{\underline{\#2}}:} The node (challenger-node) that receives a join request from a new node requests a remote attestation to verify the trustworthiness of the TEE and the loaded code ($\S$~\ref{subsec:attestation}). 
   
    \noindent{}{\bf{\underline{\#3}}:} After a successful attestation, the challenger-node shares the network encryption keys, etc., and the configuration of the membership by replying back to the join-request. Once the new joiner acknowledges that it received the configuration, the replicas are notified about the new membership. 
    %\footnote{\projecttitle{} does not make any assumption of who is in change of distributing the configuration. $\S$~\ref{subsec:attestation} explains how \projecttitle{} implements configuration distribution. However, the developer can build its own configuration and attestation service building on top of \projecttitle{}'s TEE-assisted primitives.}
    
    % and waits for \texttt{ACK} before proceeding. This handshake verifies that the joiner node indeed sent the request. The other replicas about the new recovering node. The configuration might be the nodes' IPs or the IP of a management service that knows about the system membership. %Joiner nodes and CAS communication is performed over a TLS network channel.
    %\item[3.]  and communicates with a node of the membership with a request <\texttt{JOIN\_REQ(uid)$_s$}>, \texttt{uid} is a randomly generated unique id from that node.
    %\item[4.] The recovering node marks its state as \texttt{RECOVERING} The node that receives a join request from a new node sends back a <\texttt{VERIFY\_ID\_REQ(uid)$_s$}> and waits for \texttt{ACK} before proceeding. This handshake verifies that the joiner node indeed sent the request. The other replicas about the new recovering node.
    
    \noindent{}{\bf{\underline{\#4}}:} The new node marks its state as Recovering and act as a shadow replica fetching the state of the system. If the CFT protocol allows it, joiner nodes can participate in writes while recovering. Once the replica is fully synchronized with the current state of the system, it changes its state to Normal. The replica can now execute the entire protocol. % After reading the entire applications state, the shadow replica is up-to-date and transitions to operational state, whereby it is able to serve client requests.
    %and updates the replicas (or the management service) about the membership change
%\end{itemize}

\myparagraph{Persistent storage for recovery} \projecttitle{} does not support secure recovery from persistent storage. Persistent data are susceptible to rollback attacks where the adversaries can replace the data with stale, yet valid, versions of it. Nevertheless, developers are able to support recovery from persistent (local) logs and checkpoints (if necessary) at the cost of relying on external trusted services for rollback violations detection, similarly to other systems~\cite{engraft, treaty, rote, speicher-fast}.

==> space_tricks.tex <==
% -*- root: main.tex -*-

%space left between floats.
\setlength{\floatsep}{4mm}
% space between last top float or first bottom float and the text.
\setlength{\textfloatsep}{2mm}

% space left on top and bottom of an in-text float.
\setlength{\intextsep}{0.5mm}
% space above caption
\setlength{\abovecaptionskip}{2mm}
%space below caption
\setlength{\belowcaptionskip}{0mm}

%% Change figure handling
\renewcommand{\topfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{1}

%\usepackage[small,compact,noindentafter]{titlesec}
%\usepackage[compact]{titlesec}

%\titlespacing\section{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
%\titlespacing\subsection{0pt}{4pt plus 2pt minus 2pt}{2pt plus 1pt minus 1pt}
%\titlespacing{\paragraph}{0pt}{2pt plus 0pt minus 1pt}{1.0ex}

\usepackage[inline]{enumitem}
\setlist{noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt}
\setlist[itemize]{leftmargin=*}
\setlist[enumerate]{leftmargin=*}
\setlist{itemsep=0pt,parsep=0pt}  

%\usepackage[subtle]{savetrees}
% \usepackage[moderate]{savetrees}

\usepackage{setspace}
\usepackage[margin=5pt,font={stretch=0.9}]{caption}
%\usepackage[margin=8pt,font={small,bf,stretch=0.85}]{caption}

